Boson Stars in AdS

We construct boson stars in global Anti de Sitter (AdS) space and study their stability. Linear perturbation results suggest that the ground state along with the first three excited state boson stars are stable. We evolve some of these solutions and study their nonlinear stability in light of recent work \cite{Bizon:2011gg} arguing that a weakly turbulent instability drives scalar perturbations of AdS to black hole formation. However evolutions suggest that boson stars are nonlinearly stable and immune to the instability for sufficiently small perturbation. Furthermore, these studies find other families of initial data which similarly avoid the instability for sufficiently weak parameters. Heuristically, we argue that initial data families with widely distributed mass-energy distort the spacetime sufficiently to oppose the coherent amplification favored by the instability. From the dual CFT perspective our findings suggest that there exist families of rather generic initial conditions in strongly coupled CFT (with large number of degrees of freedom) that do not thermalize in the infinite future.

==> alex.tex <==
\catcode`\@=11

%%%
%%%%%% draftcontrol
%%%%%%%%%
\expandafter\ifx\csname draftcontrol\endcsname\relax\global\def\draftcontrol{0}
\fi

%%%
%%%%%% draftdate
%%%%%%%%%
{\count255=\time\divide\count255 by 60
\xdef\hourmin{\number\count255}
\multiply\count255 by-60\advance\count255 by\time
\xdef\hourmin{\hourmin:\ifnum\count255<10 0\fi\the\count255}}
\def\draftdate{\number\month/\number\day/\number\year\ \ \ \hourmin }

%%%
%%%%%% titlepage (adapted from article.cls)
%%%%%%%%%
\newcommand\makepapertitle{\par
  \begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@1.8em{%
                \hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
     \newpage
     \global\@topnum\z@   % Prevents figures from going at top of page.
     \@makepapertitle
     \thispagestyle{empty}\@thanks
  \endgroup
  \setcounter{footnote}{0}%
  \global\let\thanks\relax
  \global\let\makepapertitle\relax
  \global\let\@makepapertitle\relax
  \global\let\@thanks\@empty
  \global\let\@author\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax
  \def\version{\let\version\@version\@gobble}
}
\def\@makepapertitle{%
  \newpage
   \ifnum\draftcontrol=1 {}
   \version\versionno
   \vskip 3em%
   \else
   \hfill\hbox to 3cm {\parbox{4cm}{\@pubnum}\hss}%
   \vskip 3em%
   \fi
   \begin{center}%
   \let \footnote \thanks
     {\LARGE {\@title}}%
     \vskip 1.5em%
     {\normalsize%\large
       \lineskip .5em%
       \begin{tabular}[t]{c}%
         \@author
       \end{tabular}\par}%
     \vskip 1.5em%
     {\@bstract}%
     \end{center}%
     \vskip 1.5em
     \@date%
   \par
}

\gdef\@pubnum{}
%\@latex@error{No \noexpand \pubnum given}\@ehc}
\def\pubnum#1{%
  \gdef\@pubnum{#1}}

\gdef\@bstract{}
\def\Abstract#1{%
  \gdef\@bstract{%
   \parbox{\textwidth-0pc}{%
   \centerline{\bf Abstract}\penalty1000%
\kern.2cm%
\noindent%\abstractfont \baselineskip=12pt
\renewcommand\baselinestretch{1.0}%
{#1}}}
}


%%%
%%%%%% pagestyle
%%%%%%%%% for body of text
%%%%%%%%%%%%
\def\ps@paper{\let\@mkboth\@gobbletwo%
     \ifnum\draftcontrol=1
    \def\@oddfoot{\hbox to \textwidth{\tiny \versionno \hfil\tiny\draftdate}%
    \hskip -\textwidth \hbox to \textwidth{\hfil\rm\thepage\hfil}}%
     \else\def\@oddfoot{\hbox to \textwidth{\hfil\rm\thepage\hfil}}
     \fi
     \let\@evenfoot\@oddfoot
}
%%%%%%%%%%%%%%%%%%

%%%
%%%%%% front vs body vs coda
%%%%%%%%%
\def\body{\clearpage
%         \pagenumbering{arabic}
          \pagestyle{paper}
    }
\newenvironment{acknowledgments}{%
\vskip 3.25ex
%\@startsection {section}{1}{\z@}%
%                                   {-3.25ex \@plus -1ex \@minus -.2ex}%
%                                   {1.5ex \@plus.2ex}%
%                                   {\normalfont\normalsize\bfseries}
\noindent {\bf Acknowledgments}
%\vskip 0in
%\noindent
}

%%%%%%%%%%%%

%%%
%%%%%% definitions for draftmode
%%%%%%%%%
%%%%%%%%%%%% versioncontrol
%%%%%%%%%%%%%%%
\def\@version#1{\ifnum\draftcontrol=1
\typeout{}\typeout{#1}\typeout{}
\vskip3mm\centerline{\hbox{\fbox{\normalsize{\tt DRAFT -- #1 -- }
                   {\draftdate}}}}\vskip3mm
\fi}
\let\version\@version
%%%%%%%%%%%% labels in math mode
%%%%%%%%%%%%%%%
\long\def\eqlabel#1{\ifnum\draftcontrol=1
                    \tag@false  % there are some problems with multline without this
                    \tag*{(\theequation) \hbox to -0.2cm{\hspace{0cm}\small{#1}\hss}}
                    \refstepcounter{equation}
                    \edef\@currentlabel{\theequation}
                    \ltx@label{#1}          % use old LaTeX \label instead of new definition
                                            % of \label in AMSLaTeX.
                    \else
                    \label{#1}
                    \fi
                    }
%%%%%%%%%%%% citations keys in bibliography (very short version of showkeys.sty)
%%%%%%%%%%%%%%%
\let\st@bibitem\@bibitem
\let\st@lbibitem\@lbibitem
\ifnum\draftcontrol=1
  \def\@bibitem#1{%
    \st@bibitem{#1}\a@@label{#1}\ignorespaces}
  \def\@lbibitem[#1]#2{%
    \st@lbibitem[#1]{#2}\a@@label{#2}\ignorespaces}
  \def\a@@label#1{%
    \gdef\a@lab{\smash{\normalfont\small#1}}
    \ifvmode
      \if@inlabel
        \global\setbox\@labels\hbox{%
          \llap{\a@lab\let\a@lab\relax
                \kern\@totalleftmargin\kern\marginparsep}%
          \box\@labels}%
      \fi
    \fi}
\fi
%%%%%%%%%%%%%%%



